Solving Aspect Category Sentiment Analysis as a Text Generation Task

Aspect category sentiment analysis has attracted increasing research attention. The dominant methods make use of pre-trained language models by learning effective aspect category-specific representations, and adding specific output layers to its pre-trained representation. We consider a more direct way of making use of pre-trained language models, by casting the ACSA tasks into natural language generation tasks, using natural language sentences to represent the output. Our method allows more direct use of pre-trained knowledge in seq2seq language models by directly following the task setting during pre-training. Experiments on several benchmarks show that our method gives the best reported results, having large advantages in few-shot and zero-shot settings.

==> abstract0.tex <==
\begin{abstract}
Aspect category sentiment analysis (ACSA) aims to predict sentiment polarities of sentences with respect to given aspect categories. To detect the sentiment toward a particular aspect category in a sentence, most previous methods first generate an aspect category-specific sentence representation for the aspect category, then predict the sentiment polarity based on the representation. These methods can not directly use the sentiment common sense knowledge in language model. To address the issue, we propose a template-based method for ACSA, treating ACSA as a language model ranking problem with a sequence-to-sequence framework, where original sentences and statement templates filled by candidate category are regarded as the source sequence and the target sequence, respectively. For inference, the model is required to classify each candidate category on the corresponding template scores. Experimental results on three public datasets demonstrate the effectiveness of our model.
\end{abstract}

==> introduction0.tex <==
\section{Introduction}

Sentiment analysis has attracted increasing attention recently. Aspect-based sentiment analysis (ABSA) is a fine-grained sentiment analysis task and includes many subtasks, two of which are aspect category detection (ACD) that detects the aspect categories mentioned in a sentence and aspect category sentiment analysis (ACSA) that
predicts the sentiment polarities with respect to the detected aspect categories. Figure \ref{fig:examples} shows an example. ACD detects the aspect categories, like, price and food, and ACSA predicts the negative and positive sentiment toward them respectively. In this work, we focus on these two tasks as well as joint task combing them.

Since a sentence usually contains one or more
aspect categories, previous studies have developed various methods for generating aspect category-specific sentence representations to detect the sentiment toward a particular aspect category in a sentence. Recently, pre-trained language models have shown their effectiveness to alleviate the effort of feature engineering for sentence encoding on the ACSA task. Because for aspect-related information may already be discarded and
aspect-irrelevant information may be retained in an
aspect independent encoder, some existing methods utilized the given aspect to guide the sentence encoding from scratch. However, These sentence encoding based models need to add new structure modules (such as classifiers) as output layer to complete category analysis. This means that we need rich training data to train the parameters of these new structure modules, which will make it difficult to achieve good performance in the resource limited category analysis. We think a suitable method is needed to use pre-trained language model directly to take advantage of the implicit sentiment common sense knowledge, and improve the transfer learning ability of the model.

\input{figures/example}

To address these issues, we investigate a template-based method for exploiting the few-shot learning potential of generative pre-trained language models, treating ACSA as a language model ranking problem with a sequence-to-sequence framework. Specifically, as shown in Figure \ref{fig:overview}, BART \cite{bart} is fine-tuned with pre-defined templates filled by corresponding labeled entities. For example, we can define templates such as ``\textit{ The sentiment polarity of $\langle{\tt given\_category}\rangle$ is $\langle{\tt polarity\_type}\rangle$}'', where $\langle{\tt polarity\_type}\rangle$ can be ``\textit{positive}'' and ``\textit{negative}'', etc. Given the sentence ``\textit{The restaurant was too expensive}'', where aspect category ``\textit{price}'' has a gold label ``\textit{negative}'', we can train BART using a filled template ``\textit{The sentiment polarity of price is negative.}'' as the decoder output for the input sentence. During inference, we enumerate all given categories in the input sentence as category candidates, classifying them into polarity based on BART scores on templates. 

The proposed method has three advantages. First,
since the joint probability ranking directly based on the language model, our method can make better use of sentiment common sense knowledge in the pre-trained language models and achieve better results in category analysis. Second, due to the good generalization ability of pre-trained models \cite{gpt3, gao2020making}, the network can effectively leverage labeled instances in the new domain for fine-tuning. Third, compared with sentence enconding based methods, our method is more robust even if the target domain and source domain have a large gap in category style without changing the parameters and structure of the output layer, and therefore allows continual learning \cite{cl1}.
% use the knowledge in the output layer and directly fine-tune new entity categories rather than equipping a new output layer. 
%As shown in Figure~\ref{fig:intro}, for each entity span, BART is trained to reconstruct the pre-defined template given the source text. During inference, we enumerate all possible spans in the sentence as name entity candidates, and classify them into the target entity types or non-entity by comparing the score of pre-defined template assigned by the language models. 

We conduct experiments in both ACD and ACSA tasks. We fine-tune our methods achieving effectiveness results on MAMS, SemEval-2014 Task3 as well as Task4 datasets, and outperforms BERT and BART baseline when it comes to zero-shot and few-shot settings. 
%Our approach outperforms the fine-tuned BERT by 25.9\%, 19.4\%, 7.8\% and 9.9\% absolute F1 respectively, when 10, 20, 50 and 100 instances per entity type are available in the target domain (MIT restaurant reviews).
% We further find that proposed methods outperform standard fine-tuning in two aspects. First, our methods need less data than fine-tuning during training on in-domain datasets. Second, our methods can efficiency make use of the knowledge learned from source data-rich datasets when transfer to target domain. 
To the best of our knowledge, we are the first to employ a generative pre-trained language model to address a ACSA/ACD problem. We release our code at \url{https://anonymous}.


\input{figures/overview}

==> tables/continual.tex <==
\begin{table}[t!]
\small
    \begin{tabular}{c|c|c|c}
        \toprule
        \multirow{2}{*}{Source} & \multicolumn{3}{c}{\textit{Rest14 + MAMS\_100}}\\
        \cmidrule{2-4}
        & Methods & Rest14 & MAMS  \\
        \midrule
        \multirow{3}{*}{MAMS} & BERT & 83.04  & 72.91  \\
         & BART & 84.27 &  73.80 \\
         & Template-based BART & 89.87  &  82.13  \\
        \bottomrule
    \end{tabular}
    \caption{\label{tab:continual}Continual learning performance on different test sets.100 indicates 100 instances for each entity types.}
\end{table}

==> tables/few_shot.tex <==
\begin{table*}[t!]
\centering
\scriptsize
\begin{tabular}{c|c|c|c|c|c|c}
\toprule
\multicolumn{7}{c}{\textit{Rest14}}\\
\midrule
    Methods & 10 & 20 & 50 & 100 & 200 & 500 \\
\midrule
     BERT classification & 38.57 & 64.75  & 68.04 & 71.22  & 77.29 & 82.93  \\
     BART classification & 50.16  & 68.96  & 72.25  & 78.21  & 82.63  & 84.79  \\
     BART generation & 82.01  & 82.63  & 83.86  & 86.02  & 86.74  & 87.87  \\
\midrule
    \multicolumn{7}{c}{\textit{MAMS}}\\ 
\midrule
%     Source & Methods & 10 & 20 & 50 & 100 & 200 & 500 \\
% \hline
     BERT classification & 40.53  & 54.61  &  58.60 & 60.93 & 61.71  & 65.48  \\
     BART classification & 46.39  & 58.82  &  60.82 & 66.70  & 68.37  & 71.03  \\
     BART generation & 62.93  & 65.70  & 69.25  & 74.03  & 77.58  & 79.02  \\
\bottomrule
\end{tabular}
\caption{\label{tab:few_shot}Few-shot ACSA performance on different test sets. 10 indicates 10 instances for each entity types.}
\vspace{-0.1cm}
\end{table*}
